Curvature-Informed SGD via General Purpose Lie-Group Preconditioners

We present a novel approach to accelerate stochastic gradient descent (SGD) by utilizing curvature information obtained from Hessian-vector products or finite differences of parameters and gradients, similar to the BFGS algorithm. Our approach involves two preconditioners: a matrix-free preconditioner and a low-rank approximation preconditioner. We update both preconditioners online using a criterion that is robust to stochastic gradient noise and does not require line search or damping. To preserve the corresponding symmetry or invariance, our preconditioners are constrained to certain connected Lie groups. The Lie group's equivariance property simplifies the preconditioner fitting process, while its invariance property eliminates the need for damping, which is commonly required in second-order optimizers. As a result, the learning rate for parameter updating and the step size for preconditioner fitting are naturally normalized, and their default values work well in most scenarios. Our proposed approach offers a promising direction for improving the convergence of SGD with low computational overhead. We demonstrate that Preconditioned SGD (PSGD) outperforms SoTA on Vision, NLP, and RL tasks across multiple modern deep-learning architectures. We have provided code for reproducing toy and large scale experiments in this paper.

==> background_short.tex <==
\section{Background}
\subsection{Notations}
We consider the problem of minimizing a loss function $f(\theta) = E_z[\ell(\theta, z)]$, where $\theta\in \mathbb{R}^n$ is the parameter vector to be optimized and $z$ is a random vector. We assume that the problem is second-order differentiable. We use $\hat{f}(\theta)$ to denote a sampled noisy evaluation of $f(\theta)$. A step of stochastic gradient descent (\sgd) with learning rate $\mu$ and an optional positive definite preconditioner $P$ is given by:
\begin{equation}
\theta_{i+1} = \theta_{i} - \mu P ,{\partial \hat{f}(\theta)}/{\partial \theta}\left.\right|_{\theta=\theta_i} \label{eq:gradprecond}
\end{equation}
where $i$ is the iteration index, $\mu>0$ is the learning rate, and $P$ typically is a variable or adaptive preconditioner.

\subsection{The Preconditioner Fitting Criterion}
We adopt the preconditioner fitting criterion proposed in \cite{psgd}, which is:
\begin{equation} \label{eq:fitting}
c(P) = E_{v}[(\nabla_v \hat{f}(\theta^{})^T P \nabla_v \hat{f}(\theta^{}) + v^T P^{-1}v]
\end{equation}
where $v$ is a random vector, $\theta^*$ is a local minimum, $\nabla_v \hat{f}(\theta^{})$ is the gradient of $\hat{f}(\theta)$ with respect to $v$, and $P$ is a positive definite preconditioner. With auto differentiation tools, we can replace the pair $(v, \nabla_v \hat{f}(\theta^{*}))$ with $(v, \hat{H}v)$, where $\hat{H}v$ is the noisy Hessian-vector product, which can be evaluated as cheaply as gradients. Criterion \eqref{eq:fitting} only has one positive definite solution, $P = (H^2 + E_v[\epsilon^2])^{-1/2}$, even for indefinite $H$, where $\epsilon = \hat{H} - H$ is a stochastic noise term. This preconditioner automatically dampens gradient noise. It is worth noting that criterion \eqref{eq:fitting} gives the same preconditioner used in equilibrated \sgd (ESGD) \cite{Dauphin15} and AdaHessian \cite{adahessian} when $P$ is diagonal.

\subsection{Preconditioners on Lie Groups}

It is natural to fit the preconditioner on a Lie group for several reasons.
First, by rewriting equation \eqref{eq:gradprecond} as
$
P^{-1/2}\theta_{i+1} = P^{-1/2}\theta_{i} - \mu ,{\partial \hat{f}(\theta)}/{\partial (P^{-1/2}\theta)}\left.\right|_{\theta=\theta_i},
$
it becomes clear that a preconditioned \sgd (\psgd)is equivalent to \sgd in a new set of coordinates defined by $\vartheta = P^{-1/2}\theta$.
This coordinate change consists of rotations and scalings, i.e., operations on the orthogonal group $O(n)$ and the group of nonsingular diagonal matrices.
We can represent this coordinate transform with matrix $Q^{-1}$, and accordingly, $P=Q^TQ$.
Thus, we pursue a variable $Q$ on the Lie group to fit this coordinate transform.

Second, \psgd can also be viewed as \sgd with transformed features when the parameters to be learned are a list of affine transform matrices \cite{psgd_affine}.
Specifically, the most commonly used feature transformations, e.g., whitening, normalization and scaling, can be represented as matrices on Lie groups.
For example, the popular batch normalization operation \cite{batchnorm} can be represented as a sparse preconditioning matrix on a Lie group where only the diagonal and last column can have nonzero values \cite{psgd_affine}. Again, Lie group arises as a natural object to work with.

Lastly, Lie groups have two properties that are particularly suitable for our task. Like any group, a certain Lie group preserves certain symmetries or invariances.
For example, with $Q\in GL^+(n, \mathbb{R})$, the general linear group with positive determinant, $\vartheta$ and $\theta$ will always have the same orientation.
This eliminates the need for damping or similar remedies to avoid degenerate solutions, since $P=Q^TQ$ is guaranteed to be always invertible.
The equivariance property of Lie groups further facilitates the preconditioner fitting.
The same group generator, i.e., the one at the identity matrix, can be used to move a preconditioner on any point of the Lie group.

The preconditioners proposed in \cite{psgd_affine} can only be applied to a list of affine transform matrix parameters.
While many machine learning models indeed consist exclusively of affine transforms and nonlinear activation functions, this is not always the case.
Additionally, it can be impractical to reparameterize many existing modules, such as a convolutional layer, into their equivalent affine transform forms.
Hence, in this paper, we propose two types of novel black box preconditioners.

==> bblgp_short.tex <==
  
\section{Black Box Lie Group Preconditioners}

\subsection{Simple Matrix Free Preconditioners}

The term `matrix free' suggests that we do not explicitly form the matrix representations. 
The Lie groups keep to be  abstract forms, i.e.,   transformations in  vector space,  $T: \mathbb{R}^n\mapsto \mathbb{R}^n$. 
The following theorem gives one systematic way to construct such sparse Lie group preconditioners. 

\emph{Proposition 1:} Let $K=\{\sigma_1, \ldots, \sigma_m\}$ be a subgroup of the permutation group $S_n$. 
Then, linear transform
$
T: \mathbb{R}^n \mapsto \mathbb{R}^n, \quad T(x|a_1, \ldots, a_m) = \sum_{i=1}^m a_i\odot \sigma_i(x)
$, forms a subgroup of $GL(n, \mathbb{R})$ parameterized with $\{a_1, \ldots, a_m\}$ if $T(\cdot|a_1, \ldots, a_m) $ is bijective, where both $a_i$ and $x$ are in $\mathbb{R}^n$.


Proposition 1 is proved by showing that   $T$ can be reduced into the direct sum of  $\lceil n/|K|\rceil$ smaller irreducible Lie groups, where $|K|$ is the order of  $K$. 
We list a few prominent examples in the below. 

\emph{Example 1}: the group of invertible diagonal matrices. We must have $K=\{e\}$ if $|K|=1$, where  $e$ is the identity element of $S_n$, i.e., $e(x)=x$. 
Then, $T$ simply has a diagonal matrix representation, i.e., $T(x|a_1) = {\rm diag}(a_1) x$. 
Criterion \eqref{eq:fitting} gives the preconditioner in  ESGD \cite{Dauphin15} and AdaHessian \cite{adahessian} as a special case when $P$ is on this group. 

\emph{Example 2}: the group of X-shape matrices. 
Let $K=\{e, \sigma_f\}$, where $\sigma_f$ denotes the flipping permutation. 
Then, we can show that 
\begin{align*}
T(\cdot|a, b)  T(\cdot|u, v) & =T(\cdot|a\odot u + b \odot \sigma_f(v), a\odot v + b \odot \sigma_f(u)) \\
T^{-1}(\cdot|a, b) & = T(\cdot|  {\sigma_f(a)\oslash c , -b\oslash c})
\end{align*}
where $c = a\odot \sigma_f(a) - b\odot \sigma_f(b)$. 
Clearly, such transforms form a Lie group if invertible, i.e., no element of $c$ is zero. 
The matrix representation of this $T$ only has nonzero diagonal and anti-diagonal elements, thus the name X-shape matrix. 


\emph{Example 3}: the butterfly matrix \cite{butterfly}. For an even $n$, subgroup $K=\{ e, s_{n/2} \}$ induces  a Lie group whose representations are invertible butterfly matrices, where $s_{n/2}$ denotes circular shifting by $n/2$ positions.  This group of matrices are the building blocks of the Kaleidoscope matrices \cite{butterfly}. 

\emph{Example 4}: the plain dense invertible matrix. The group $GL(n, \mathbb{R})$ can be recovered by letting  $K=\{ e, s_{1}, \ldots, s_{n-1} \}$, where  $s_{i}$ denotes circular shifting by $i$ positions.  

The group $GL(n, \mathbb{R})$ is too expensive  for large scale problems. 
The group of diagonal matrices, also called the Jacobi preconditioner in its matrix form, is sparse enough, but  empirically  shown to be less effective without the help of momentum for certain machine learning problems.  
We are mostly interested in the cases with $2\le |K|\le 4$.
These Lie groups are  sparse enough, yet simple enough to derive their inverse  manually, and at the same time can significantly accelerate the convergence of \sgd by shortcutting gradients separated far away in positions. 


\subsection{Low Rank Approximation Preconditioner}

Low-rank approximation (LRA) is a standard technique for processing large-scale matrices. However, commonly adopted forms of positive definite low-rank approximation, such as $P=\rho I + UU^T$, cannot always be factorized as $P=Q^TQ$ for certain Lie groups, where $\rho>0$ is a small positive number. Additionally, this form of approximation is not effective for reducing eigenvalue spread. In many real-world problems, the Hessian has a few very large and very small eigenvalues, i.e., tails on both ends of the spectrum. However, all the eigenvalues of $P$ in this form are lower bounded by $\rho$, meaning that it can only fit one tail of the spectrum when rank$(U)\ll n$.  

For this reason, we propose a new low-rank approximation with form $Q= \rho (I + UV^T)$, where $\rho$ is not necessarily small nor positive, and $U$ and $V$ have $r$ columns with $r\ll n$. To justify this form of approximation, we need to show two facts. First, preconditioner $P=Q^TQ$ with this form can fit both tails of the spectra of Hessian \om{why is this important.}. Second, we can update this preconditioner on Lie groups.


\emph{Proposition 2:} Preconditioner $P=Q^TQ$ with $Q =\rho( I+UV^T)$ can have positive eigenvalues arbitrarily larger than $\rho^2$ and arbitrarily smaller than $\rho^2$ with proper $U$ and $V$. 

\emph{Proposition 3:}  If $\rho\ne 0$ and $(I+V^TU)^{-1}$ or $(I+U^TV)^{-1}$ exists, $A_V(\rho, U)=\rho(I+UV^T)$ defines a subgroup of $GL(n, \mathbb{R})$ parameterized with $\rho$ and $U$. Similarly, $A_U(\rho,V)=\rho(I+UV^T)$ defines another  subgroup of  $GL(n, \mathbb{R})$ parameterized with $\rho$ and $V$. 

We skip the proofs here. Proposition 2 can be shown to be true just by checking the simplest case with $n=2$ and $r=1$. 
Proposition 3 can be shown to be true by verifying the four requirements of being a Lie group. Notably, the Lie algebra  is closed, e.g., 
$
<U_1V^T, U_2V^T >  =  (U_1V^TU_2 - U_2V^TU_1)V^T
$ on Lie group $A_V(U)$, where $<\cdot>$ is the Lie bracket. 
The condition that $(I+V^TU)^{-1}$ or $(I+U^TV)^{-1}$ exists is  to ensure that $I+UV^T$ is invertible as shown by the Woodbury matrix identity. 
The rotation ambiguity, i.e., $I+UV^T=I+UR(VR)^T$ for any $RR^T=I$, can be removed by assuming $I+V^TU$ having the Schur decomposition form, if necessary. 


==> emperical_new.tex <==
\section{Empirical Results}

==> emperical_short.tex <==
\section{Emperical Results}
We evaluate the performance of the PSGD algorithm on a diverse set of tasks, including vision, natural language processing (NLP), and reinforcement learning (RL) \cite{MNIST,CIFAR10,lstm,GPT,PTB,OWT,PPO,GYM}. In the domain of computer vision, we evaluate the algorithm's performance on the MNIST \cite{MNIST} and CIFAR10 \cite{CIFAR10} datasets (see Table \ref{tab:table1},\ref{tab:table2}). Additionally, we consider several variants of the CIFAR10 dataset, including those with noisy labels, adversarial attacks, and class imbalances (see Table \ref{tab:cifar10_modified}).0-

For NLP tasks, we study the use of LSTMs \cite{lstm} and GPT-2 style transformers \cite{GPT}, on various text corpora, including the Penn Treebank \cite{PTB}, the complete works of Shakespeare, and the Open Web Text (OWT) dataset \cite{OWT} (see Table \ref{tab:lstm}, \ref{tab:nanoGPT}). In the RL setting, we consider a Proximal Policy Optimization (PPO) \cite{PPO} applied to the HalfCheetah and RoboWalker environments using OpenAI's gym environments \cite{GYM} (see Fig. \ref{fig:RL}).

Once we have established the performance of PSGD on standard benchmarks, we consider specially designed tasks to gain insight into how curvature information may help solve problems compared to first-order methods.

We conduct uncertainty and forgetability analysis on classifiers trained with first and second-order optimizers, collecting statistics on entropy and margin. We also evaluate the robustness of solutions found by different optimizers on a version of CIFAR10 dataset with label noise that shifts during training, gaining insights into transfer learning applications. Additionally, we examine the delayed XOR problem introduced in \cite{lstm} to understand the strengths and limitations of different optimization methods.

\input{resnet_short.tex}

\input{language_modeling_short.tex}

\input{RL.tex}

\input{explore_first_vs_second_short.tex}


==> explore/figures.tex <==
\begin{figure}[ht]
\vspace{-4mm}
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{Figs/noisy_lucky.png} 
    \caption{\textbf{Noisy Label CIFAR-10} }
    \label{fig:stuborn}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{Figs/blur_plot.png}
    \caption{\textbf{Nero-Plasticity}}
    \label{fig:neuroplastic}
  \end{subfigure}
  \vspace{1mm}
   \caption{a) Solutions found by SGD are harder to optimize compared to PSGD. Note for SGD we used a lucky initialization (see \ref{luckyinit}). The blue and yellow dotted line are the average accuracy of PSGD and SGD 
 after 100 epochs respectivly. b) Removing the blur-deficit at epoch 100, PSGD is be more neuro-plastic compared to SGD, achieving better train and test performance.}
  % \vspace{-1mm}
\end{figure}

==> explore/stuborn.tex <==
\textbf{Stubborn Solutions of First Order Optimizers}\label{stuborn}
From the previous examples, we learned that first-order optimizers tend to heavily overfit certain data points, reducing entropy. In the case of noisy labels, this often results in pure memorization where the network achieves the training accuracy of PSGD on the train set, but only $10\%$ accuracy on the test dataset with an average confidence of $99.9\%$. To better understand the stubbornness of SGD solutions, we consider the \textit{lucky initialization,} which resulted in a test accuracy of $77\%$ under noisy label conditions.
Here, we examine a transfer learning problem, where a ResNet18 was trained on noisy data for 100 epochs and then on clean labels for another 100 epochs. This simulates a real-world distributional shift where noisy labels may be refined throughout training, leading to a distributional shift. We compare neural networks trained with each optimizer, as well as those that changed optimizers after 100 epochs of training.

As seen in Fig \ref{fig:stuborn}, PSGD finds a flexible solution when given noisy labels. This is seen since when we correct the labels both PSGD and SGD can reach an accuracy of 92.42\%. In contrast, the solution found by SGD seems to be stubborn since when we correct the noisy labels, PSGD then SGD reaches an accuracy of 91.7\% and SGD then PSGD has an accuracy of 88\%. This shows the importance of curvature information in the early periods of training.  


\begin{figure}[ht]
\vspace{-4mm}
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{Figs/noisy_lucky.png} 
    \caption{\textbf{Noisy Label CIFAR-10} }
    \label{fig:stuborn}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{Figs/blur_plot.png}
    \caption{\textbf{Nero-Plasticity}}
    \label{fig:neuroplastic}
  \end{subfigure}
  \vspace{1mm}
   \caption{a) Solutions found by SGD are harder to optimize compared to PSGD. Note for SGD we used a lucky initialization (see \ref{luckyinit}). The blue and yellow dotted line are the average accuracy of PSGD and SGD 
 after 100 epochs respectivly. b) Removing the blur-deficit at epoch 100, PSGD is be more neuro-plastic compared to SGD, achieving better train and test performance.}
\end{figure}

Intuitively, first-order methods cause NNs to dedicate parameters to memorizing some data points, unnecessarily reducing entropy. When memorization occurs given incorrect labels, it may be difficult to reshape
the NN when the labels are corrected, leading to the loss in generalization accuracy seen in Fig \ref{fig:stuborn}. In contrast, as PSGD finds a less certain or suborn solution in the first stage of training, either optimizer can then reshape the NN to their liking in the second stage. 

We believe the noisy-label and neuro-plasticity results have strong applicability to transfer learning and coreset selection \cite{adacore}, particularly in scenarios where the training distribution changes during training. Recently, \cite{osawa2022asdl} demonstrated that the affine Lie group variant of PSGD outperforms other optimizers when fine-tuning a ResNet18 and ViT \cite{ViT} on CIFAR10 that were pre-trained on ImageNet \cite{imagenet}.

==> explore_first_vs_second_back.tex <==
\subsection{Towards Understanding Second Order Optimizers}

With the performance distinctions between PSGD and SGD now apparent, we aim to conduct a series of simple experiments to provide further insight into the reasons behind the stark contrast in the nature of the two optimizers.

\textbf{Uncertainty Analysis}
We train a standard ResNet18 on CIFAR10 with PSGD and SGD, and after 200 epochs we check the entropy over the softmax-logits and miss-classification margin \cite{toneva2018empirical} of both NNs. 
We see in Table \ref{table:entropy} that PSGD has higher entropy and a lower margin of classification compared to first-order optimizers. This very low minimum entropy of first-order optimizers may be interpreted as a form of overfitting. Intuitively, some data points (low entropy/unforgettable) have information that is easily memorized by NNs, giving up network capacity learning points that do not improve generalization. 
Conversely, we observe that PSGD never becomes overly certain about any data point, with the minimum entropy being six orders of magnitude larger than that of SGD. Similar trends can be observed in the mean and maximum entropy values. In terms of margin, PSGD on average has a $95\%$ certainty level for classifications, while SGD has a staggering $99.9\%.$ 
From these statistics, we believe standard first and second order optimizers can push NNs into a dangerous regime of overconfidence which given clean labels can reduce their generalization capacity with the potential of catastrophic forgetting. In the scenario where a network is given noisy labels (or imaginably poisoned points), training with first-order methods may lead to memorization of the training set with hindered to no generalization capacity as seen in Table \ref{tab:cifar10_modified} column Noisy Final. 

PSGD's higher entropy and lower margins are indications of a larger exploration of the parameter space, more diverse solutions, and a lack of memorization.
Suggesting that PSGD is able to better balance the trade-off between overfitting and underfitting, without memorizing points. 

\textbf{Forgettability Statistics and Learning}
We revisit \cite{toneva2018empirical}'s forgettability experiments, which found that one can prune $30\%$ of the CIFAR-10 train samples without loss of generalization. The study found that a point's utility for generalization increases as it is learned and then subsequently forgotten during training, regardless of the optimizer or architecture used. Essentially, forgettability ordering shows which data points a NN uses to define high-dimensional boundaries akin to support vectors. We investigate whether the performance difference between PSGD and SGD's generalization performance can be attributed to this forgettability ordering.
Furthermore, \cite{toneva2018empirical} revealed a strong correlation between forgettable points and high margin, which we explore by examining the expected forgettability ordering of the two optimizers and whether pruning points based on their orderings affects performance.

We train the ResNet18 three times pruning CIFAR10 by 25k, 35k, and 45k points based on each optimizer's forgettability score. 
Table \ref{tab:forgetting} shows that points PSGD focuses on based on forgettability ordering outperform that of SGD. When we limit the dataset to only the 5k most forgettable datapoints, we see PSGD is able to outperform SGD by nearly 14\%. 


SGD and PSGD exhibit fundamentally different importance orderings, which is evident from the significant generalization gap observed when training on pruned datasets using these orderings at various degrees. We find that PSGD and SGD have a statistically significant correlation between their forgettability orderings, but the strength of the correlation is weak (Spearman coefficient of 0.02 and a p-value of $p=1$x$10^{-12}$). This indicates that the nature of training observed through forgettability is different for PSGD compared to first-order optimizers. 

Furthermore, we see a strong correlation coefficient of 0.75 and 0.60 between a low forgetability score and low entropy score with a p-value of $p=0$ for PSGD and SGD respectively (see Fig \ref{fig:fvu}). Hence, PSGD does a better job of shaping the NN to focus on the highly forgettable points that are important for generalization while not becoming overconfident on the easy unforgettable points giving up too much capacity, unnecessarily pushing the parameters away from initialization reducing generalization ability \cite{quanquan} (see \ref{highlowhsubsets}). Note while \cite{toneva2018empirical} shows that forgettable points are more important for generalization for supervised learning, very recently \cite{omead_lebm} showed low entropy points are the more important points for learning in the unsupervised, semi-supervised, and generative model setting. See Table \ref{highlowhsubsets} showing generalization gap training low and high entropy points and how it affects the distance from initialization. 


\begin{table}
\vspace{-8mm}
\begin{minipage}{0.44\textwidth}
\centering
\captionof{table}{Uncertainty Statistics: PSGD's higher uncertainty leads to better generalization and less over-fitting. 
}
\label{table:entropy}
\scalebox{0.73}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{NTK} & \multicolumn{3}{c}{\textbf{Entropy}}   & \multicolumn{3}{c}{\textbf{Margin}} \\ \midrule
        & Min       & Mean & Max & Min   & Mean  & Max  \\
PSGD     & 0.139       & 0.260 & 1.545 & 0.144  & 0.956  & 0.994  \\
SGD      & 7x$10^{-7}$ & 0.01 & 0.8975 & 0.3925  & 0.999  & 1   \\ 
Adam      & 1.5x$10^{-7}$ & 0.009 & 0.8645 & 0.3625  & 0.999  & 1   \\ 
AdaHessian      & 1x$10^{-6}$ & 0.05 & 0.8843 & 0.4225  & 0.999  & 1   \\ 
\bottomrule

\end{tabular}
}
\end{minipage}
\hfill
\begin{minipage}{0.44\textwidth}
\centering
\captionof{table}{Forgetting statistics for CIFAR10 on ResNet18. PSGD finds better forgettability statistics outperforming SGD.}
\vspace{-2mm}
\label{tab:forgetting}
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Forgetting} & \textbf{50k} & \textbf{25k} & \textbf{15k} & \textbf{5k} \\ \midrule
PSGD     & 96.65   & 95.83  & 94.95  & 56.46  \\
SGD      &  96.21   & 95.56  & 93.7   & 42.48  \\ \bottomrule
\end{tabular}
\end{minipage}
\vspace{-6.6mm}
\end{table}



\textbf{Stubborn Solutions of First Order Optimizers}
From the previous examples, we learned that first-order optimizers tend to heavily overfit certain data points, reducing entropy. In the case of noisy labels, this often results in pure memorization where the network achieves the training accuracy of PSGD on the train set, but only $10\%$ accuracy on the test dataset with an average confidence of $99.9\%$. To better understand the stubbornness of SGD solutions, we consider the \textit{lucky initialization,} which resulted in a test accuracy of $77\%$ under noisy label conditions.
Here, we examine a transfer learning problem, where a ResNet18 was trained on noisy data for 100 epochs and then on clean labels for another 100 epochs. This simulates a real-world distributional shift where noisy labels may be refined throughout training, leading to a distributional shift. We compare neural networks trained with each optimizer, as well as those that changed optimizers after 100 epochs of training.

As seen in Fig \ref{fig:stuborn}, PSGD finds a flexible solution when given noisy labels. This is seen since when we correct the labels both PSGD and SGD can reach an accuracy of 92.42\%. In contrast, the solution found by SGD seems to be stubborn since when we correct the noisy labels, PSGD then SGD reaches an accuracy of 91.7\% and SGD then PSGD has an accuracy of 88\%. This shows the importance of curvature information in the early periods of training.  


Intuitively, first-order methods cause NNs to dedicate parameters to memorizing some data points, unnecessarily reducing entropy. When memorization occurs given incorrect labels, it may be difficult to reshape
the NN when the labels are corrected, leading to the loss in generalization accuracy seen in Fig \ref{fig:stuborn}. In contrast, as PSGD finds a less certain or suborn solution in the first stage of training, either optimizer can then reshape the NN to their liking in the second stage. 

\begin{figure}[ht]
\vspace{-4mm}
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{Figs/noisy_lucky.png} 
    \caption{\textbf{Noisy Label CIFAR-10} }
    \label{fig:stuborn}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{Figs/blur_plot.png}
    \caption{\textbf{Nero-Plasticity}}
    \label{fig:neuroplastic}
  \end{subfigure}
  \vspace{1mm}
   \caption{a) Solutions found by SGD are harder to optimize compared to PSGD. Note for SGD we used a lucky initialization (see \ref{luckyinit}). The blue and yellow dotted line are the average accuracy of PSGD and SGD 
 after 100 epochs respectivly. b) Removing the blur-deficit at epoch 100, PSGD is be more neuro-plastic compared to SGD, achieving better train and test performance.}
\end{figure}
\textbf{PSGD Preserves Neuro-Plasticity}
Recently, \cite{neuroplastic} studied the phenomenon  of neuro-plasticity in NNs. The presents an different lense to our stubborn solution hypothesis. They found that NNs exhibit a critical learning period, during which if a learning deficit is not removed, the NN becomes unable to learn effectively. To simulate this deficit, CIFAR10 images are blurred for the first half of training, after which the deficit is removed. Following \cite{neuroplastic}, we used an exponential learning rate decay. To investigate the impact of optimization on neuro-plasticity we compare SGD and PSGD. We find that PSGD retains neuro-plasticity outperforming SGD by 6 and 3\% on test and train sets seen in Fig \ref{fig:neuroplastic} and Table \ref{tab:cifar10_modified}. 

We believe the noisy-label and neuro-plasticity results have strong applicability to transfer learning and coreset selection \cite{adacore}, particularly in scenarios where the training distribution changes during training. Recently, \cite{osawa2022asdl} demonstrated that the affine Kronecker variant of PSGD outperforms other first and second-order optimizers when fine-tuning a ResNet18 and ViT \cite{ViT} on CIFAR10 that were pre-trained on ImageNet \cite{imagenet}. 

\textbf{Understanding long term dependence via Delayed XOR Problem}
%
We consider the delayed XOR problem proposed in the LSTM paper \cite{lstm}. 
The task is to predict the XOR relation of $a$ and $b$ scattered randomly and far away in a long sequence. 
This problem is challenging for many architectures and optimizers because it cannot be ``partially solved'' since memorizing either $a$ or $b$ alone does not help to predict XOR$(a, b)$. 
We consider solving this problem with standard RNNs and LSTMs optimized using SGD, AdaBelief, Adan, AdaHessian, Hessian Free, Shampoo, KFAC, and PSGD at different sequence lengths. 
The success rates for each optimizer are shown in Table \ref{tab:xor}. 
In our experiments, we find that PSGD LRA is the only method that can solve the XOR problem past the length of 32 with an RNN. Furthermore, LSTMs show no benefit to RNNs without using curvature information for the XOR problem. Finally, PSGD optimizes an RNN to solve the XOR problem better than any of the other methods using an LSTM. These result hint, that while increasing model parameters and architecture complexity may boost performance, the choice of optimizer may be more important for certain problems. See \ref{xorrank} for rank analysis. 


\begin{table}[h]
% \vspace{-4mm}
\centering
\caption{Delayed XOR problem at length 32,55,64, and 112 averaged over 10 runs. An RNN optimized with PSGD outperforms other optimizers with an RNN or LSTM. This hints that the choice of optimizer may be more important than network architecture.}
\scalebox{0.65}{
% \begin{table}[]
\begin{tabular}{c|cccccccccccccccc}
\hline
\textbf{XOR} &
 \multicolumn{2}{c}{\textbf{PSGD LRA}} &
 \multicolumn{2}{c}{\textbf{AdaHessian}} &
 \multicolumn{2}{c}{\textbf{KFAC}} &
 \multicolumn{2}{c}{\textbf{HessianFree}} &
 \multicolumn{2}{c}{\textbf{Shampoo}} &
 \multicolumn{2}{c}{\textbf{SGD}} &
 \multicolumn{2}{c}{\textbf{AdaBelief}} &
 \multicolumn{2}{c}{\textbf{Adan}} \\ % \hline
Length &
RNN &
 LSTM &
RNN &
 LSTM &
RNN &
 LSTM &
 \multicolumn{1}{l}{RNN} &
 \multicolumn{1}{l}{LSTM} &
 \multicolumn{1}{l}{RNN} &
 \multicolumn{1}{l}{LSTM} &
RNN &
 LSTM &
RNN &
 LSTM &
RNN &
 LSTM \\ \hline
\textbf{32} & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
\textbf{55} & 1 & 1 & 0 & 1 & 0 & 0 & 0 & 0.6 & 0 & 0.8 & 0 & 0 & 0 & 0 & 0 & 0 \\
\textbf{64} & 1 & 1 & 0 & 0.8 & 0 & 0 & 0 & 0 & 0 & 0.6 & 0 & 0 & 0 & 0 & 0 & 0 \\
\textbf{112} & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0
\end{tabular}
}
\label{tab:xor}
\vspace{-7mm}
\end{table}


==> explore_first_vs_second_short.tex <==
\subsection{Towards Understanding Second Order Optimizers}

Now that we have some clear numerical disctinctions between PSGD and SGD we consider some simple experiments to provide insight on how/why the nature of the optimizers are so different. 


\textbf{Uncertainty Analysis}
We trained ResNet18 on CIFAR10 with PSGD and SGD, and evaluated the entropy and classification margin of both methods after 200 epochs \cite{toneva2018empirical}. Table \ref{table:entropy} shows that PSGD has higher entropy and lower margin compared to SGD and Adam-style optimizers. This suggests that first order optimizers may overfit by exploiting easy-to-learn datapoints, creating deep basins in the loss landscape that unnecessarily limit the NN's capacity. PSGD, on the other hand, avoids overconfidence and promotes exploration, leading to more diverse solutions. These observations are supported by statistics on mean and maximum entropy. Furthermore, we found that PSGD's more cautious approach to classification yields better generalization, as seen in experiment Table \ref{tab:cifar10_modified} column Noisy Final.

\begin{table*}[ht]
    \begin{center}
    \caption{PSGD is a lot less certain which leads to better generalization and less overfitting. All variances were less than two significant figures }
    
    \label{table:entropy}
    \begin{tabular}{@{}lcccccc@{}}
    \toprule
    \textbf{CIFAR10 -- NTK} & \multicolumn{3}{c}{\textbf{Entropy}}            & \multicolumn{3}{c}{\textbf{Margin}} \\ \midrule
                                   & Min                            & Mean  & Max    & Min         & Mean      & Max       \\
    PSGD LRA + M                   & 0.139                          & 0.260 & 1.545  & 0.144       & 0.956     & 0.994     \\
    SGD                        & 7.5x$10^{-7}$ & 0.01  & 0.8975 & 0.3925      & 0.999     & 1         \\ \bottomrule
    \end{tabular}

    \end{center} 
\end{table*}

\textbf{Forgettability Statistics and Learning}
In this section, we revisit the forgettability experiments that shed light on the composition of datasets in machine learning \cite{toneva2018empirical}. The study showed that a point's utility for generalization increases as it is learned and then forgotten during training. The results were consistent across various architectures and first-order optimizers. We investigate whether forgettability and its ordering can demonstrate a performance difference between the two optimizers, given that PSGD exhibits a significant difference in behavior compared to SGD with respect to entropy and margin.

We obtain forgettability orderings by training a ResNet18 five times using PSGD and SGD with different seeds. The points are then ordered based on their forgettability score, which is the average number of times they were forgotten after being correctly classified by the network. Previous research \cite{toneva2018empirical} has shown that pruning points with a low forgettability score can remove approximately $30\%$ of the CIFAR10 dataset without reducing generalization accuracy. The results also indicate that points with high forgettability scores are essential for generalization, except for mislabeled points.

Once we have the forgettability scores for each optimizer, we retrain the ResNet18 three times, pruning CIFAR10 by 25k, 35k, and 45k points based on forgettability score. The results show that PSGD's forgettability ordering outperforms that of SGD, as shown in Table \ref{tab:forgetting}. When we limit the dataset to only the 5k most forgettable datapoints, we see PSGD outperforming SGD by nearly $14\%.$

SGD and PSGD exhibit fundamentally different importance orderings, which is evident from the significant generalization gap observed when training on pruned datasets using these orderings at various degrees. We find that PSGD and SGD have a statistically significant correlation between their forgettability orderings, but the strength of the correlation is weak (Spearman coefficient of 0.02 and a p-value of $p=1\times10^{-12}$). This indicates that the nature of training observed through forgettability is different for PSGD compared to first-order optimizers.

Intuitively, we believe that PSGD is able to focus on highly forgettable points that are important for generalization without becoming overconfident on easy unforgettable or low forgettability points, giving up too much capacity.




\begin{table}[ht]
\vspace{-4mm}
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{CIFAR10 -- Forgetting} & \textbf{50k} & \textbf{25k} & \textbf{15k} & \textbf{5k} \\ \midrule
PSGD LRA + M                   &    96.65          & 95.83        & 94.95        & 56.46       \\
SGD                        &     96.21         & 95.56        & 93.7         & 42.48       \\ \bottomrule
\end{tabular}
\caption{Results for optimizing a ResNet18. We see that PSGD was able to find better forgettability statistics, as well as learn from the subset of data better than SOTA optimizer.  }
\vspace{-5mm}
\label{tab:forgetting}
\end{table}

\textbf{Stubborn Solutions of First Order Optimizers}

First order optimizers tend to overfit certain datapoints, pushing the network parameters far from initialization. This lack of generalization is exemplified by the "gifted kid syndrome" where the network achieves high training accuracy but poor test accuracy. To investigate the stubbornness of solutions found by SGD, we consider a transfer learning problem where a ResNet18 was trained for 100 epochs on noisy data and then for another 100 epochs on clean labels. We compare the performance of NNs trained with individual optimizers as well as changing optimizers after 100 epochs.

Fig. \ref{fig:stuborn} shows that PSGD finds a flexible solution when given noisy labels, as evidenced by its ability to reach $92.42\%$ accuracy when the labels are corrected. In contrast, SGD's solution appears stubborn, achieving only $91.7\%$ accuracy when the labels are corrected. This can be explained by the fact that first order methods create deep grooves in the loss landscape, reducing entropy and making it difficult to reshape the network when given corrected labels.

These results have implications for transfer learning and coreset selection, where the training distribution may change throughout training.
\begin{figure}
    % \vspace{-5mm}
    \centering
    \includegraphics[width=0.35\textwidth]{Figs/stuborn.png}
    \caption{We can clearly see the solutions that SGD results in is harder to optimize. }
    \label{fig:stuborn}
    \vspace{-4mm}
\end{figure}

\textbf{Understanding long term dependence via Delayed XOR Problem}

We investigate long-term dependence via the delayed XOR problem \cite{lstm}. The problem involves predicting XOR relation between two scattered and distant inputs in a long sequence. The task is challenging since memorizing each input alone does not help predict the output. We use standard RNNs and LSTMs with various optimizers (SGD, AdaBelief, Adan, AdaHessian, Hessian Free, Shampoo, KFAC, and PSGD) at sequence lengths of 32, 55, 64, and 112. We perform ten runs per optimizer for 100,000 iterations or until convergence. Results are shown in Table \ref{tab:xor}. PSGD LRA ($r=10$) is the only method that can solve the XOR problem past a length of 32 with an RNN. Furthermore, using curvature information does not provide any benefit to LSTMs over RNNs for the XOR problem. Lastly, PSGD optimizes an RNN better than any of the other methods using an LSTM. These results suggest that the choice of optimizer may be more crucial to solving certain problems than increasing model parameters or complexifying architecture.

We use the full-rank version of PSGD \cite{psgd_affine} to solve the XOR problem with an RNN past a delay of 128. We also test the effect of rank on convergence on the XOR problem using an RNN with low-rank approximations ($r=0,1,2,5,$ and $10$). Results are plotted in Fig.~3. This example shows that while the diagonal preconditioner struggles, a low-order Hessian approximation works well for preconditioning.

\begin{table}[h]
\centering
\scalebox{0.65}{

\begin{tabular}{c|cccccccccccccccc}
\hline
\textbf{XOR} &
  \multicolumn{2}{c}{\textbf{PSGD LRA}} &
  \multicolumn{2}{c}{\textbf{AdaHessian}} &
  \multicolumn{2}{c}{\textbf{KFAC}} &
  \multicolumn{2}{c}{\textbf{HessianFree}} &
  \multicolumn{2}{c}{\textbf{Shampoo}} &
  \multicolumn{2}{c}{\textbf{SGD}} &
  \multicolumn{2}{c}{\textbf{AdaBelief}} &
  \multicolumn{2}{c}{\textbf{Adan}} \\ \hline
\textbf{Length} &
  \textbf{RNN} &
  \textbf{LSTM} &
  \textbf{RNN} &
  \textbf{LSTM} &
  \textbf{RNN} &
  \textbf{LSTM} &
  \multicolumn{1}{l}{\textbf{RNN}} &
  \multicolumn{1}{l}{\textbf{LSTM}} &
  \multicolumn{1}{l}{\textbf{RNN}} &
  \multicolumn{1}{l}{\textbf{LSTM}} &
  \textbf{RNN} &
  \textbf{LSTM} &
  \textbf{RNN} &
  \textbf{LSTM} &
  \textbf{RNN} &
  \textbf{LSTM} \\ \hline
\textbf{32}  & 1 & 1 & 1 & 1   & 1 & 1 & 1 & 1 & 0 & 1   & 1 & 1 & 1 & 1 & 1 & 1 \\
\textbf{55}  & 1 & 1 & 0 & 1   & 0 & 0 &  0 & 0.6  & 0 & 0.8 & 0 & 0 & 0 & 0 & 0 & 0 \\
\textbf{64}  & 1 & 1 & 0 & 0.8 & 0 & 0 &  0 & 0  & 0 & 0.6 & 0 & 0 & 0 & 0 & 0 & 0 \\
\textbf{112} & 1 & 1 & 0 & 0   & 0 & 0 & 0 & 0 & 0 &  0   & 0 & 0 & 0 & 0 & 0 & 0
\end{tabular}
}
\caption{Solving the delayed XOR problem at length 32,55,64, and 112 using various first and second order optimizers. We see that PSGD with an RNN is able to outperform other optimizers using either an RNN or LSTM. This hints that the choice of optimizer may be more important than network architecture.}
\label{tab:xor}
\end{table}


\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{Figs/xor.eps}
\caption{Success rate over ten runs in solving the XOR problem with a simple RNN and LRA preconditioners of orders $0,1,2,5$ and $10$.  Higher is better.  }
\end{figure}



==> future.tex <==
\section{Future Work}

\begin{enumerate}
    \item Combine Xmat and UVd, update Xmat much more often that UVd to get the best of both worlds. 
    \item Update UVd like is done in LBFGS
    \item Assume we have some Affine network instead of calculating full curvature per layer cauculate UVd per layer
    \item Assume we have some Affine network it would be nice to do Kron over each layer but also tie them together using UVd or Xmat
    \item So a rank 1 update like LBFGS may be best done in this way via sketching using Frequency Directions... https://arxiv.org/pdf/2302.03764.pdf \om{this looks like a good way to do coresets as well. OMP and Facility location gave sparse outputs. FL's points can be better i feel and OMP was too sparce}
\end{enumerate}

==> intro_short.tex <==
\section{Introduction}
Optimizing machine learning models with millions of free parameters is challenging due to the limitations of conventional convex optimization algorithms. While algorithms like Broyden-Fletcher-Goldfarb-Shanno (BFGS) and its limited-memory version, LM-BFGS, conjugate gradient (CG), and Hessian-free (HF) optimization \cite{Martens12} are suitable for small-scale convex problems, they are not ideal for large-scale stochastic optimization problems that arise in machine learning. The reliance on the line search step is one of the main reasons for this. ML models often define cost functions as expectations, which can only be evaluated through Monte Carlo (MC) sampling averages, resulting in large variances. Optimizers that rely on line search can have convergence issues due to this. Recently, K-BFGS and KFAC\cite{KBFGS,kfac} have foregone the line search step in favor of damping, but this introduces extra hyperparameters.

Large sample sizes can cause new issues, including increased generalization gaps and low computational efficiency. While \sgd is a highly efficient optimizer for most ML problems, it may converge slowly once the solution is located in a basin of attraction for problems with a large eigenvalue spread. Regret optimizers like RMSProp and Adam \cite{adam} converge faster but may generalize worse on many problems. This paper focuses on providing \sgd with a good preconditioner to accelerate its convergence without undermining its generalization capacity.

In this paper, we propose using Lie groups as a tool for preconditioner fitting, which involves applying a series of small transforms via multiplication with $I + \mu G$, where $\mu$ is a small scalar and $G$ is the group generator. A Lie group is a friendly object to work with since moving a preconditioner around any point on a Lie group behaves similarly to moving it around the identity element of the group, i.e., the identity matrix $I$. This is known as the equivariance property of a Lie group. The preconditioner fitting criterion proposed in \cite{psgd} is used, which is more general and gradient noise-robust than deterministic methods. The preconditioner is fit online with another ``gradient descent" algorithm, without making the preconditioner fitting problem more difficult and computationally expensive than the original parameter learning problem.

While recent curvature-aware optimization methods have shown good empirical results in Deep Learning, they require damping, line search, or regret and hence are susceptible to pitfalls that do not affect PSGD \cite{osawa2022asdl}.


==> notation.tex <==

\newcommand{\tsn}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\usepackage{xcolor}
\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
% \hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}

%--------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{result}{Result}
\newtheorem{problem}{Problem}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{remark}[subsection]{Remark}
\newtheorem{remarks}[subsection]{Remarks}
\newtheorem{example}[subsection]{Example}


%% TT's definitions
\newcommand\tr{{{\operatorname{trace}}}}
%\newcommand{\eps}{\varepsilon}
\newcommand{\epsr}{\varepsilon_R}
\newcommand{\mur}{\mu_R}

\newcommand{\tin}[1]{\|{#1}\|_{\ell_\infty}}
\newcommand{\tone}[1]{\|{#1}\|_{\ell_1}}
\newcommand{\eb}{\vct{e}}
\newcommand{\bdd}{\delta}
\newcommand{\be}{\epsilon}
\newcommand{\Scp}{\mathcal{S}_+}
\newcommand{\Scn}{\mathcal{S}_-}
\newcommand{\el}{L}
%\newcommand{\vc}[1]{{\text{vect}(#1)}}
\newcommand{\alpb}{\zeta}
\newcommand{\alpbb}{(\la -\eta\bp^2/2)\bn}
\newcommand{\gam}{{\gamma}}
\newcommand{\KB}{\bar{K}}
\newcommand{\xw}{\x_{\w}}
\newcommand{\xv}{\x_{\vb}}
\newcommand{\xu}{\x_{\ub}}
\newcommand{\xvt}[1]{\x_{\vb_{#1}}}
\newcommand{\xvtt}[1]{\x_{\vb,#1}}
\newcommand{\xwt}[1]{\x_{#1,\w}}
\newcommand{\xws}[1]{\x_{#1,\ws}}
\newcommand{\xs}{\x_{\ws}}
\newcommand{\yst}{\hat{\y}}
\newcommand{\eig}{\text{eigvec}}
\newcommand{\hu}{h}
%\newcommand{\ru}{r}
\newcommand{\pbar}{{{\bar{p}}}}
\newcommand{\pbd}{p}
\newcommand{\bp}{\beta}
\newcommand{\bn}{\alpha}
\newcommand{\lay}[1]{{\vct{k}}^{(#1)}}
\newcommand{\lah}[1]{{\vct{\hat{k}}}^{(#1)}}
\newcommand{\lan}{\vct{k}}
\newcommand{\rest}{{\bf{r}}}
\newcommand{\dcp}{\vct{d}^{\text{cnn}}}
\newcommand{\fcp}{\vct{g}^{\text{CNN}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\nrest}{\bar{n}}
%\newcommand{\vs}{{\vspace*{-4pt}}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\prox}{{{\text{\bf{prox}}}}}
\newcommand{\cov}{{{\text{\bf{cov}}}}}
\newcommand{\ex}{{{\text{\bf{ex}}}}}
\newcommand{\modu}{{{\text{{mod}}}}}
\newcommand{\map}{{{\text{\bf{map}}}}}
\newcommand{\var}[1]{{{\text{\bf{var}}}}[#1]}
\newcommand{\func}[1]{{f_{\text{CNN}}}(#1)}
\newcommand{\funh}[1]{{{\hat{f}}_{\text{CNN}}}(#1)}
\newcommand{\funcp}[1]{{f'_{\text{cnn}}}(#1)}
\newcommand{\funcw}[1]{{{{f}}'_{\text{cnn}}}(#1)}
\newcommand{\dev}{{{\text{\bf{dev}}}}}
\newcommand{\meas}{{{\text{\bf{mean}}(\sigma)}}}
\newcommand{\nn}{\nonumber}
\newcommand{\la}{\lambda}
\newcommand{\A}{{\mtx{A}}}
\newcommand{\amp}{\alpha_{\text{cnn}}}
\newcommand{\bt}{\bigotimes}
%\newcommand{\bt}{\times}
\newcommand{\robt}[1]{\bigotimes_{\ell=1}^D{#1}_{\ell}}
\newcommand{\robtu}[1]{\bigotimes_{\ell=1}^D{#1}^{(\ell)}}
\newcommand{\bd}{\bigodot}
\newcommand{\kal}{\prod_{i=1}^{D-1}\tn{\lay{i}}}
%\newcommand{\kall}[1]{\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\kall}[1]{1_{\lan #1}}
\newcommand{\lall}[1]{{\order{\lip_{\lan #1}}}}%{L^{#1}\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\lell}[1]{{\lip}_{\lan #1}}
\newcommand{\bell}[1]{{{{\beta}}}_{\lan #1}}
\newcommand{\Ub}{{\mtx{U}}}
\newcommand{\Ubb}{{\mtx{U}}}
\newcommand{\V}{{\mtx{V}}}
\newcommand{\ten}{(\{\vb_\ell\}_{\ell=1}^D)}
\newcommand{\uten}{(\{\ub_\ell\}_{\ell=1}^D)}
\newcommand{\ken}{(\{\lay{i}\}_{i=1}^D)}
\newcommand{\B}{{{\mtx{B}}}}
\newcommand{\alx}{{{\alpha_\X}}}
\newcommand{\aly}[1]{{{\alpha_{\X_{#1}}}}}
\newcommand{\Ib}{{{\mtx{I}}}}
\newcommand{\Xbin}{{{\mtx{B}}}}
\newcommand{\Gbin}{{{\mtx{S}}}}
\newcommand{\xbin}{{{\mtx{b}}}}
\newcommand{\Sb}{{{\mtx{S}}}}
\newcommand{\Gb}{{\mtx{G}}}
\newcommand{\ymean}{{\bar{\y}(\w;\text{avg})}}
\newcommand{\yavg}{{{y}_{\text{avg}}}}
\newcommand{\ravg}[1]{{{r}_{{\text{avg}}}(#1)}}
\newcommand{\fmean}{{\funcw{\w;\text{avg}}}}
\newcommand{\diag}{\text{diag}}
\newcommand{\out}{\text{out}}
\newcommand{\linest}{\text{lin}}
\newcommand{\inp}{\text{in}}
\newcommand{\inh}{\hat{\text{in}}}
\newcommand{\sexp}{subexponential }
\newcommand{\Lc}{{\cal{L}}}
\newcommand{\Jc}{{\cal{J}}}
\newcommand{\Dc}{{\cal{D}}}
%\newcommand{\smn}{\s_{\min}}
\newcommand{\btd}{{\bt_{\ell=1}^D d_\ell}}
\newcommand{\Ro}{{\cal{RO}}}
\newcommand{\PC}{{\cal{PC}}}
\newcommand{\Vc}{{\cal{V}}}
\newcommand{\Pb}{{\mtx{P}}}
\newcommand{\Tb}{{\mtx{T}}}
\newcommand{\Kba}{{\vct{k}}_{\text{all}}}
\newcommand{\Qb}{{\mtx{Q}}}
\newcommand{\rng}{\gamma}
\newcommand{\Cb}{{\mtx{C}}}
\newcommand{\Eb}{{\mtx{E}}}
\newcommand{\Hb}{{\mtx{H}}}
\newcommand{\Gc}{{\cal{G}}}
\newcommand{\F}{{\mtx{F}}}
\newcommand{\diff}{{\text{diff}}}
\newcommand{\La}{{\boldsymbol{{\Lambda}}}}
%\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\sigmap}{\phi'}
\newcommand{\sigmal}[1]{\sigma^{(#1)}}
\newcommand{\sigmalp}[1]{\sigma'^{(#1)}}
\newcommand{\sigmaa}{\sigma'_{\text{all}}}
\newcommand{\sigmai}[1]{\sigma'_{\text{all},#1}}
\newcommand{\bSi}{{\boldsymbol{{\Sigma}}}}
\newcommand{\bSit}{{\boldsymbol{{\tilde{\Sigma}}}}}
\newcommand{\bSih}{{\boldsymbol{{\hat{\Sigma}}}}}
\newcommand{\bmu}{{\boldsymbol{{\mu}}}}
\newcommand{\bv}{{\boldsymbol{{v}}}}
\newcommand{\bw}{{\boldsymbol{{w}}}}
\newcommand{\Db}{{\mtx{D}}}
\newcommand{\db}{{\vct{d}}}
\newcommand{\oneb}{{\mathbb{1}}}
\newcommand{\onebb}{{\mathbf{1}}}
\newcommand{\Iden}{{\mtx{I}}}
\newcommand{\M}{{\mtx{M}}}
\newcommand{\stuff}{{\theta}}
\newcommand{\gm}{\gamma_m}
\newcommand{\distas}{\overset{\text{i.i.d.}}{\sim}}
\newcommand{\order}[1]{{\cal{O}}(#1)}
\newcommand{\torder}[1]{\tilde{\cal{O}}(#1)}
\newcommand{\rmax}[1]{{\bf{r}_{\max}(#1)}}
\newcommand{\rbmax}[1]{{\bf{\bar{r}}_{\max}(#1)}}
\newcommand{\rmin}[1]{{\bf{r}_{\min}(#1)}}
\newcommand{\smn}[1]{{\sigma_{\min}(#1)}}
\newcommand{\smx}[1]{{\sigma_{\max}(#1)}}
\newcommand{\z}{{\vct{z}}}
\newcommand{\zb}{{\bar{\z}}}
\newcommand{\tn}[1]{\|{#1}\|_{\ell_2}}
\newcommand{\tti}[1]{\|{#1}\|_{2,\infty}}
\newcommand{\bad}{{\bar{d}}}
\newcommand{\Dp}{{D^+}}
\newcommand{\tf}[1]{\|{#1}\|_{F}}
\newcommand{\te}[1]{\|{#1}\|_{\psi_1}}
\newcommand{\tsub}[1]{\|{#1}\|_{\psi_2}}
\newcommand{\tsut}[1]{\|{#1}\|_{\psi_{2/3}}}
\newcommand{\tsup}[1]{\|{#1}\|_{\psi_a}}
\newcommand{\dist}[1]{\text{dist}(#1)}
%\newcommand{\supp}[1]{\text{supp}(#1)}
\newcommand{\cone}[1]{{\text{cone}(#1)}}
\newcommand{\paf}{\partial f(\x)}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ccb}{\bar{\mathcal{C}}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\btrue}{\bbeta_{true}}
\newcommand{\bteta}{\boldsymbol{\theta}}
\newcommand{\bTeta}{\boldsymbol{\Theta}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\ddelta}{{\boldsymbol{\delta}}}
\newcommand{\babeta}{{\bar{\beta}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Mc}{\mathbb{S}^{dr-1}}
\newcommand{\pa}{{\partial}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\pol}{^\circ}
\newcommand{\vb}{\vct{v}}
\newcommand{\Jb}{\mtx{J}}
\newcommand{\vbl}{\vct{v}^{\text{lin}}}
\newcommand{\fb}{\vct{f}}
\newcommand{\ib}{{\bf{i}}}
\newcommand{\hib}{{\bf{\hat{i}}}}
\newcommand{\all}{{\text{all}}}
%\newcommand{\vh}{\vct{\hat{v}}}
\newcommand{\vbb}{\vct{\bar{v}}}
\newcommand{\Xb}{\mtx{\bar{X}}}
\newcommand{\abb}{\mtx{\bar{a}}}
\newcommand{\cb}{\mtx{c}}
\newcommand{\bbb}{\mtx{\bar{b}}}
\newcommand{\w}{\vct{w}}
\newcommand{\Wp}{\mtx{W}^\dagger}
\newcommand{\ob}{\mtx{o}}
\newcommand{\obh}{\mtx{\hat{o}}}
\newcommand{\wh}{{\hat{\mtx{w}}}}
\newcommand{\li}{\left<}
%\newcommand{\ri}{\right>}
\newcommand{\s}{\vct{s}}
%\newcommand{\ab}{\vct{a}}
\newcommand{\bb}{\vct{b}}
\newcommand{\ub}{{\vct{u}}}
\newcommand{\ubb}{\bar{\vct{u}}}
\newcommand{\h}{\vct{h}}
\newcommand{\hh}{{\vct{h}}}
\newcommand{\g}{{\vct{g}}}
\newcommand{\ii}{{\vct{i}}}
\newcommand{\zm}[1]{{\text{{\bf{zm}}}(#1)}}
\newcommand{\dd}{{\vct{d}}}
\newcommand{\ddt}{{\vct{d}}_\tau}
\newcommand{\Zb}{\mtx{Z}}
\newcommand{\hf}{\hat{f}}
\newcommand{\corrCA}{\rho_\Cc(\M)}
\newcommand{\corr}[1]{{\bf{cor}}(#1)}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Fc}{\mathcal{F}}


%%YP's macros
%\newcommand{\qqq}[1]{{\textcolor{red}{?{#1}?}}}
\newcommand{\rbb}{\vct{\bar{r}}}
%\newcommand{\rh}{\vct{\hat{r}}}
%\newcommand{\rt}{\vct{\tilde{r}}}

\newcommand{\qqq}[1]{{\textcolor{black}{{#1}}}}
\newcommand{\ihere}{{\textcolor{red}{I AM HERE! }}}
\newcommand{\mat}[1]{{\text{mat}\left(#1\right)}}
\newcommand{\gb}{\bar{\g}}
\newcommand{\bs}{\bar{s}}
\newcommand{\cgain}{\alpha_{\text{CNN}}}
\newcommand{\cgainp}{\tn{\E_{\x\sim\Nn(0,\Iden)}[\gcnn{}]}}
\newcommand{\gcnn}[1]{{\vct{g}}_{\text{cnn}#1}}
\newcommand{\ccorr}{\rho_{\text{cnn}}}
\newcommand{\kb}{\vct{k}}
\newcommand{\xh}{\hat{\x}}
\newcommand{\yh}{\hat{\y}}
\newcommand{\xbr}{\bar{\h}}
\newcommand{\xdr}{\tilde{\x}}
\newcommand{\m}{\vct{m}}
\newcommand{\xt}{\tilde{\x}}
\newcommand{\gh}{\hat{\g}}
\newcommand{\gt}{\tilde{\g}}
\newcommand{\wb}{\bar{\w}}
\newcommand{\lip}{L}
\newcommand{\mipp}{L_{\max}}
\newcommand{\mupp}{\bar{\mu}_{\max}}
\newcommand{\mapp}{\mu}
\newcommand{\tcnn}{{\mtx{T}}_{\text{cnn}}}
\newcommand{\lcnn}{{\mtx{L}}_{\text{CNN}}}
\newcommand{\lipa}{{L}}
\newcommand{\smo}{S}
\newcommand{\SM}{{{\bf{S}}}_{L,\kb}}
\newcommand{\SMB}{{{\bf{\bar{S}}}}_{L,\kb}}
\newcommand{\Ws}{\W^\star}
\newcommand{\ws}{{\w^\star}}
\newcommand{\wss}{{\w^\star}}
\newcommand{\yp}[1]{\textcolor{red}{ #1}}
\newcommand{\zeronorm}[1]{\left\|#1 \right\|_0}
\newcommand{\unorm}[1]{\left\|#1 \right\|_u}
\newcommand{\ynorm}[1]{\left\|#1 \right\|_{\bar{y}}}
\newcommand{\onetwonorm}[1]{\left\|#1\right\|_{1,2}}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\onenorm}[1]{\left\|#1\right\|_{\ell_1}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\Dnorm}[1]{\left\|#1\right\|_{D}}
\newcommand{\oneinfnorm}[1]{\left\|#1\right\|_{1,\infty}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\avg}[1]{\left< #1 \right>}

\newcommand{\lipp}{\prod_{\ell=1}^D \twonorm{\vct{k}^{(\ell)}}}

\renewcommand{\d}{\mathrm{d}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\rotd}{\text{R1TD}}
\newcommand{\nntd}{\text{DeepTD}}
\newcommand{\x}{\vct{x}}
\newcommand{\rb}{\vct{r}}
\newcommand{\rt}{\tilde{\vct{r}}}
\newcommand{\rbt}{\vct{r}(\vct{\theta})}
\newcommand{\y}{\vct{y}}
\newcommand{\ybh}{\vct{\hat{y}}}
\newcommand{\W}{\mtx{W}}
\newcommand{\bgl}{{~\big |~}}

%--------------

% EJC's macros

%\definecolor{emmanuel}{RGB}{255,127,0}
%\newcommand{\ejc}[1]{\textcolor{emmanuel}{EJC: #1}}

\newcommand{\p}{{\vct{p}}}
\newcommand{\Kb}{{\mtx{K}}}
\newcommand{\somelog}{16\Kb\log (\Kb)}
\newcommand{\somelg}{\Kb\log (\Kb)}
\newcommand{\pb}{{\vct{p}}}
\newcommand{\qb}{{\vct{q}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
%\newcommand{\Var}{\textrm{Var}}
\newcommand{\sgn}[1]{\textrm{sgn}(#1)}
\renewcommand{\P}{\operatorname{\mathbb{P}}}
%\newcommand{\E}{\operatorname{\mathbb{E}}}
%\newcommand{\var}{\operatorname{\mathbf{var}}}

\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\grad}[1]{{\nabla\Lc(#1)}}
\newcommand{\gradf}[1]{{\nabla f(#1)}}
\newcommand{\hessf}[1]{{\nabla^2f(#1)}}
\newcommand{\gradw}[1]{{\nabla{\Lc}(#1)}}
\newcommand{\grd}[2]{{\nabla\Lc_{#1}(#2)}}
\newcommand{\e}{\mathrm{e}}
\renewcommand{\i}{\imath}

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

% MS's macros

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
\newcommand{\restrict}[1]{\big\vert_{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\OpId}{\mathcal{I}}
\newcommand{\bz}{B}
\newcommand{\cp}{R_{p}}
\newcommand{\cs}{\nu}

\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Imag}{\operatorname{Im}}

\newcommand{\piyp}{\pi'_1(\vct{y})}
\newcommand{\piy}{\pi_1(\vct{y})}
\newcommand{\piar}{\pi_1(\vct{a}_r)}
\newcommand{\piarp}{\pi'_1(\vct{a}_r)}
\newcommand{\set}{{\cal{F}}}
\newcommand{\des}{{\x_0}}

\newcommand{\Pc}{{\cal{P}}}
\newcommand{\X}{{\mtx{X}}}
\newcommand{\Y}{{\mtx{Y}}}
\newcommand{\Vb}{{\mtx{V}}}
\newcommand{\Vh}{\hat{{\mtx{V}}}}
\newcommand{\Vbd}{{\mtx{V}^\dagger}}
\newcommand{\Rb}{{\mtx{R}}}


\newcommand{\MS}[1]{\textcolor{blue}{MS: #1}}
\newcommand{\MST}[1]{\textcolor{red}{#1}}
\newcommand{\SO}[1]{\textcolor{darkgreen}{SO: #1}}

%\usepackage{chngcntr}
%\numberwithin{equation}{section} 

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}
\newenvironment{proofsk}{\noindent {\bf Proof sketch} }{\endprf\par}


\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           \nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}

\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}

\newcommand{\red}{\textcolor{red}}
\newcommand{\gi}{\ab_{\gamma_i}}
\newcommand{\ang}{\text{ang}}
\newcommand{\ham}[2]{{\|#1,#2\|_H}}


==> pl_proof.tex <==
In this section, we first prove that $\psgd$ achieves a linear convergence rate under non-convex settings with proper assumptions.

\subsection{Convergence Analysis}
We assume the risk function $\Lc$ satisfies the following conditions:
\begin{assumption}\label{as:diff}
$\Lc(\theta)$ is twice continuously differentiable.
\end{assumption}

\begin{assumption}\label{as:smooth}
$\ell_i(\theta)$ is $\beta$-smooth for $1\leq i \leq N$, $\beta > 0$: 
$\forall \theta_1, \theta_2$, $||\nabla\ell_i(\theta_2)-\nabla\ell_i(\theta_1) ||\leq \beta ||\theta_2-\theta_1||$.
\end{assumption}

\begin{assumption}\label{as:pl}
$\Loss(\btheta)$ is $\lambda$-PL: it satisfies Polyak-Lojasiewicz (PL) condition for a constant $\lambda > 0$: $\norm{\grad{L}(\btheta)}^2 \geq \lambda\Loss(\btheta)$.
\end{assumption}

The smooth condition in AS \ref{as:smooth} is commonly used in analyzing convergence in practical optimization. 
In addition, noting that compared to typical strong convexity assumptions, the PL condition in AS \ref{as:pl} applies to a more general setting \citep{PL}.
Strong convexity implies the PL condition, but not vice versa. In AS \ref{as:pl}, we relax the constraint and only require the gradient variance to be lower bounded. 

With the assumptions, we present the convergence theorem as follows. Proofs are deferred to Appendix \ref{appx:proof}.
\begin{theorem}\label{theorem:convergence}
Assume AS \ref{as:diff}-\ref{as:pl} hold at each iteration $t$ of \method{} with mini-batch input $\tX_t$ where each sample is randomly sampled from  $\mathcal{X}$ with replacement, then the expectation of $\Loss(\btheta_{t})$ satisfies
\begin{center}
    $E_{\tX_{t}}[\Loss(\btheta_{t})] \leq \alpha_{t-1} E_{\tX_{t-1}}[\Loss(\btheta_{t-1})]$,
\end{center}
where $\alpha_{t-1} = 1-\eta_{t-1}\lambda\xi + \eta_{t-1}^2\Lambda^2\Xi^2$. $\xi$ and $\Xi$ denotes the lower and upper bound of the $\HI$.% and the expectations are with respect to the minibatches $\mathcal{S}_t$ and $\mathcal{S}_{t+1}$. %With $0<\eta_t < \frac{1}{2\lambda\xi}$, SLIM-QN converges to minimum $\mathcal{L}_{\otheta}$ in a linear rate.
\end{theorem}

By choosing $\eta_{t-1}$ such that $\alpha_{t-1} < 1$, \method{} converges at a linear rate. 
The convergence rate matches the best rate in stochastic QN optimizations. It is worth mentioning that no convergence rate beyond linear is observed in stochastic L-BFGS optimizations.
Theorem~\ref{theorem:convergence} is not aimed to push the theoretical convergence limit. Instead, it investigates the effects of momentum in the Hessian and block-diagonal approximation.
In addition, as mentioned earlier, Theorem~\ref{theorem:convergence} also applies to convex settings, as strong convexity implies $\norm{\grad{L}(\btheta)}^2$ is lower bounded by $\Loss(\btheta)$ for an appropriate $\lambda > 0$ and hence AS \ref{as:pl} holds.



==> resnet_back.tex <==
\subsection{CIFAR-10 and Friends on ResNet18}

We examine the effectiveness of the PSGD optimizer in classifying CIFAR10-derived datasets using a ResNet18 and find it outperforms the SoTA optimizer SGD. Once the optimizers are tuned on ResNet18 with the CIFAR10 dataset, we do not change them for the rest of the experiments.


\input{resnet/standard}
\input{resnet/skip}

\textbf{Modified CIFAR10} 

Next, we evaluate the performance of SGD and PSGD on three variations of the CIFAR10 image classification task using ResNet18: class imbalance, noisy training labels, and adversarial generalization. These variations provide a rigorous test for the generalization ability of optimizers. We maintain the hyperparameters from our previous experiments on the ResNet18 CIFAR10 dataset for a fair comparison between the optimizers.

\input{resnet/imb}

\input{resnet/noisy}

\input{resnet/adv}

\begin{table*}
    \vspace{-10mm}
    \caption{Test Accuracy of RN18 on diverse CIFAR10 derived tasks with (P)SGD, Adam \& Apollo (2nd order).}    
    \vspace{-2mm}
    \begin{center}
    \label{tab:cifar10_modified}
    \vspace{-2mm}
    \scalebox{0.83}{
    \begin{tabular}{@{}llllllll@{}}
    \toprule
    CIFAR10 & Standard      & No Shortcut   & Class Imb & Noisy Final   & Noisy Best     & Adversarial &  Blur Deficit  \\ \midrule
    PSGD (Ours)  & $95.49_{0.08}$ (5.5hrs)&$ 95.27_{0.09} $& $87.16_{0.85} $ & $82.63_{0.11}$ & $82.63_{0.11}$  & $85.17_{0.04} $  & $89.51_{0.12}$\\
    SGD (SoTA)     & $95.47_{0.14}$ (4.5hrs) & $94.66_{0.16} $& $ 86.32_{0.84} $& $18.7_{33.75}$& $73.975_{5.65}$ & $83.82_{0.18}$ & $83.51_{0.15}$ \\ 
    Adam       & $93.15_{0.02}$ (4.5hrs)& $92.70_{0.02}$ & $83.18_{1.2}$ &$72.47_{2.17}$ & $74.47_{1.06}$ & $82.26_{0.49}$ & $82.62_{0.015}$  \\
    Apollo     & $90.59_{0.252}$ (5hrs) & $92.00_{0.20} $ & $78.23_{1.3}$ & $67.71_{1.49}$& $72.58_{0.92}$ & $73.9_{0.57}$ & $79.25_{0.46}$  \\
    \bottomrule
\end{tabular}
}
    \vspace{-2mm}
\end{center}
\end{table*}

